Why are inner planets not inclined?

Poincar\'e's work more than one century ago, or Laskar's numerical simulations from the 1990's on, have irrevocably impaired the long-held belief that the Solar System should be stable. But mathematical mechanisms explaining this instability have remained mysterious. In 1968, Arnold conjectured the existence of "Arnold diffusion" in celestial mechanics. We prove Arnold's conjecture in the planetary spatial $4$-body problem as well as in the corresponding hierarchical problem (where the bodies are increasingly separated), and show that this diffusion leads, on a long time interval, to some large-scale instability. Along the diffusive orbits, the mutual inclination of the two inner planets is close to $\pi/2$, which hints at why even marginal stability in planetary systems may exist only when inner planets are not inclined. More precisely, consider the normalised angular momentum of the second planet, obtained by rescaling the angular momentum by the square root of its semimajor axis and by an adequate mass factor (its direction and norm give the plane of revolution and the eccentricity of the second planet). It is a vector of the unit $3$-ball. We show that any finite sequence in this ball may be realised, up to an arbitrary precision, as a sequence of values of the normalised angular momentum in the $4$-body problem. For example, the second planet may flip from prograde nearly horizontal revolutions to retrograde ones. As a consequence of the proof, the non-recurrent set of any finite-order secular normal form accumulates on circular motions -- a weak form of a celebrated conjecture of Herman.

==> coordinates.tex <==
Consider four point masses in space, interacting via gravitational attraction in the sense of Newton. Denote by $m_j$ the mass, by $x_j \in \mathbb{R}^3$ the position, and by $y_j \in \mathbb{R}^3$ the linear momentum of body $j$ for each $j=0,1,2,3$. This system is described by the flow of the Hamiltonian function
\begin{equation} \label{eq_4bpham}
H= \sum_{0 \leq j \leq 3} \frac{y_j^2}{2m_j} - \sum_{0 \leq i < j \leq 3} \frac{m_i m_j}{\| x_j - x_i \|}.
\end{equation}
Hamilton's equations of motion give a system of 24 differential equations. It is well-known that this system has (at least) 10 integrals of motion: the integral $H$ corresponds to conservation of energy; 6 integrals correspond to the motion of the barycenter (translational symmetry); and 3 integrals correspond to conservation of angular momentum (rotational symmetry). By making suitable changes of coordinates we can make these integrals visible, thus reducing the equations of motion. First, we pass to Jacobi coordinates to perform the symplectic reduction by translational symmetry, and then use Deprit coordinates to reduce by rotational symmetry.

\subsubsection*{Reduction by Translational Symmetry}
Let
\begin{equation}
M_j = \sum_{i=0}^j m_i, \quad \sigma_{ij} = \frac{m_i}{M_j},
\end{equation}
and define the Jacobi coordinates $(q_j,p_j) \in \mathbb{R}^3 \times \mathbb{R}^3$ for $j=0,1,2,3$ by
\begin{equation}
\begin{cases}
q_0 = x_0 \\
q_1 = x_1 - x_0 \\
q_2 = x_2 - \sigma_{01} \, x_0 - \sigma_{11} \, x_1 \\
q_3 = x_3 - \sigma_{02} \, x_0 - \sigma_{12} \, x_1 - \sigma_{22} \, x_2
\end{cases}
\quad
\begin{cases}
p_0 = y_0 + y_1 + y_2 + y_3 \\
p_1 = y_1 + \sigma_{11} \, y_2 +\sigma_{11} \, y_3 \\
p_2 = y_2 + \sigma_{22} \, y_3 \\
p_3 = y_3.
\end{cases}
\end{equation}

\begin{figure}[h]
  \centering
  \begin{tikzpicture}
    \draw [->] (0,0) node[anchor=north east] {$O$}
    -- (1,1) node[anchor=north west] {$q_0$}
    -- (2,2) node[anchor=west] {$x_0$};
    \draw [->] (2,2)
    -- (1.5,2.5) node[anchor=north east] {$q_1$}
    -- (1,3) node[anchor=south east] {$x_1$};
    \draw [->] (1.5,2.5)
    -- (2,4) node[anchor=south east] {$q_2$}
    -- (2.5,5.5) node[anchor=south] {$x_2$};
    \draw [->] (2,4)
    -- (3.5,4.5) node[anchor=south east] {$q_3$}
    -- (6.5,5.5) node[anchor=west] {$x_3$};
  \end{tikzpicture}
  \caption{Jacobi coordinates}
  \label{fig:Jacobi}
\end{figure}

This is a symplectic change of coordinates, and the variable $q_0$ does not appear in the Hamiltonian~\eqref{eq_4bpham}. The reduced phase space has coordinates $(q_j,p_j)_{j=1,2,3}$, and, without loss of generality, we may restrict to $p_0=0$. Thus write
\begin{equation}
H = F_{\mathrm{Kep}} + F_{\mathrm{per}}
\end{equation}
where
\begin{equation}
F_{\mathrm{Kep}} = \sum_{j=1}^3 \left( \frac{p_j^2}{2 \mu_j} - \frac{\mu_j M_j}{\| q_j \|} \right)
\end{equation}
and
\begin{align}
F_{\mathrm{per}} ={}& \sum_{j=2}^3 \frac{\mu_j M_j}{\| q_j \|} - \frac{m_0 \, m_2}{\| q_2 + \sigma_{11} \, q_1 \|} - \frac{m_0 \, m_3}{\| q_3 + \sigma_{22} \, q_2 + \sigma_{11} \, q_1 \|} - \frac{m_1 \, m_2}{\| q_2 - \sigma_{01} \, q_1 \|}  \\
& - \frac{m_1 \, m_3}{\| q_3 + \sigma_{22} \, q_2 + (\sigma_{11} - 1) \, q_1 \|} - \frac{m_2 \, m_3}{\| q_3 + (\sigma_{22} - 1) \, q_2 
% + (\sigma_{12} + \sigma_{11} \, \sigma_{22} - \sigma_{11}) \, q_1
\|}
\end{align}
with the reduced masses $\mu_j$ defined by
\begin{equation}
\mu_j^{-1} = M_{j-1}^{-1} + m_j^{-1} \quad (j=1,2,3).
\end{equation}
The function $F_{\mathrm{Kep}}$ is an integrable Hamiltonian describing the motion of 3 uncoupled \emph{Kepler problems}, and $F_{\mathrm{per}}$ is the so-called \emph{perturbing function}.

\subsubsection*{Assumptions and Reduction by Rotational Symmetry}

In this paper, we assume that each term of $F_{\mathrm{Kep}}$ is negative, so each of the 3 uncoupled Keplerian trajectories is elliptical. We assume that the orbit of body 2 is far away from the orbits of the first two bodies. We assume moreover that the orbit of body 3 lies far from the orbits of the first 2 bodies, in a range dictated by the position of body 2. More precisely, if we denote by $a_j$ the semimajor axis of the $j^{\mathrm{th}}$ Keplerian ellipse, our assumptions are:
\begin{equation} \label{eq_assumption1}
\begin{dcases}
O(1) = a_1 \ll a_2  \to \infty \\
a_2^{\frac{11}{6}}  \ll a_3 \ll a_2^2.
\end{dcases}
\end{equation} 
The purpose of these assumptions is twofold. First, the fact that $a_1 \ll a_2 \ll a_3 \ll a_2^2$ implies that the three mean anomalies are the fastest three angles, and so we can average out these three angles (see below in this section). Second, the fact that $a_2^{11/6} \ll a_3$ implies both that the first two terms in the expansion of the secular Hamiltonian come from the quadrupolar Hamiltonian of bodies 1 and 2, and that the first nontrivial term in the Melnikov potential comes from the octupolar Hamiltonian of bodies 1 and 2 (see later).

We are in a near-integrable setting, as $F_{\mathrm{per}}$ is smaller than $F_{\mathrm{Kep}}$. Indeed, denote by $\zeta_{j}$ the angle between $q_j$ and $q_{j+1}$ for $j=1,2$, and denote by $P_n$ the Legendre polynomial of degree $n$. Our assumptions imply that $\| q_1 \| \ll \| q_2 \| \ll \| q_3 \|$. Therefore we can write the perturbing function as 
\begin{equation}
F_{\mathrm{per}} = F_{\mathrm{per}}^{12} + F_{\mathrm{per}}^{23} + O \left( \frac{\| q_1 \|^2}{\| q_3 \|^3} \right)
\end{equation}
where
\begin{align}
F_{\mathrm{per}}^{12} ={}& \frac{\mu_2 M_2}{\| q_2 \|} - \frac{m_0 \, m_2}{\| q_2 + \sigma_{11} \, q_1 \|} - \frac{m_1 \, m_2}{\| q_2 - \sigma_{01} \, q_1 \|} \\
={}& - \frac{\mu_1 m_2}{\| q_2 \|} \sum_{n=2}^{\infty} \tilde{\sigma}_{1,n} P_n (\cos \zeta_{1}) \left( \frac{\| q_1 \|}{\| q_2 \|} \right)^n \label{eq_perfn12}
\end{align}
is the perturbing function from the 3-body problem (see \cite{fejoz2016secular}, for example), and where 
\begin{equation} \label{eq_perfn23}
F_{\mathrm{per}}^{23} = - \frac{\mu_2 m_3}{\| q_3 \|} \sum_{n=2}^{\infty} \tilde{\sigma}_{2,n} P_n (\cos \zeta_{2}) \left( \frac{\| q_2 \|}{\| q_3 \|} \right)^n
\end{equation}
with
\begin{equation}
\tilde{\sigma}_{1,n} = \sigma_{01}^{n-1} + (-1)^n \sigma_{11}^{n-1}, \quad \tilde{\sigma}_{2,n} = (\sigma_{02} + \sigma_{12})^{n-1} + (-1)^n \sigma_{22}^{n-1}.
\end{equation}

We now pass to Deprit coordinates $(\ell_j, L_j, \gamma_j, \Gamma_j, \psi_j, \Psi_j)_{j=1,2,3}$ (see Appendix~\ref{sec:app:Deprit}). In these coordinates the Keplerian Hamiltonian becomes
\begin{equation}
F_{\mathrm{Kep}} = - \sum_{j=1}^3 \frac{\mu_j^3 M_j^2}{2 L_j^2}
\end{equation}
and so the mean anomalies $\ell_j$ undergo a rigid rotation with frequency $\sqrt{\frac{M_j}{a_j^3}}$, while all other variables remain fixed. Moreover  the variables $\psi_3, \Psi_2, \Psi_3$ are integrals of motion for the full 4-body problem (due to conservation of angular momentum), and so the Hamiltonian does not depend on $\Psi_3, \psi_2, \psi_3$. %See \cite{pinzari2015canonical} for a complete description of the reduction by rotational symmetry in these coordinates.

\subsubsection*{The Averaging Procedure and the Secular Hamiltonian}

It can be seen in equations \eqref{eq_perfn12}, \eqref{eq_perfn23} that $F_{\mathrm{per}}^{12}$, $F_{\mathrm{per}}^{23}$ are of order $O \left(\frac{1}{a_2^{3}} \right)$, $O \left( \frac{a_2^2}{a_3^{3}} \right)$ respectively. Therefore our assumption \eqref{eq_assumption1} implies that the mean anomalies $\ell_j$ have faster frequencies than the other angles, and moreover that the frequencies of the mean anomalies are of different orders. As a result we can apply the normal form theory (see \cite{fejoz2002quasiperiodic,zhao2014quasi}): we may construct an arbitrary number $k$ of non-resonant normal forms and find a change of coordinates close to the identity in order to obtain the Hamiltonian 
\begin{equation}\label{eq_4bphamafterave}
F = F_{\mathrm{Kep}} + F_{\mathrm{sec},k} +O \left(\left(\frac{1}{a_2} \right)^{k+1}, \, \frac{a_2^k}{a_3^{k+1}} \right)
\end{equation}
where $F_{\mathrm{sec},k}$ is the \emph{secular Hamiltonian} of order $k$, defined by 
\begin{equation} \label{eq_secularhamiltoniandef}
F_{\mathrm{sec},k} = F_{\mathrm{sec},k}^{12} + F_{\mathrm{sec},k}^{23}  + O \left( \frac{1}{a_3^3} \right)
\end{equation}
with
\begin{equation} \label{eq_secularhamiltonian12}
F_{\mathrm{sec},k}^{12} = \frac{1}{(2 \pi)^2} \int_{\mathbb{T}^2} F_{\mathrm{per}}^{12} \, d \ell_1 \, d \ell_2 + O \left( \frac{1}{a_2^{9/2}}  \right), 
\end{equation}
and
\begin{equation} \label{eq_secularhamiltonian23}
 F_{\mathrm{sec},k}^{23} = \frac{1}{(2 \pi)^2} \int_{\mathbb{T}^2} F_{\mathrm{per}}^{23} \, d \ell_2 \, d \ell_3 + O \left( \frac{a_2^4}{a_3^{9/2}} \right).
\end{equation}

Now, the first term in the expansions \eqref{eq_perfn12}, \eqref{eq_perfn23} after averaging is called the \emph{quadrupolar} Hamiltonian (with respect to bodies 1 and 2, and with respect to bodies 2 and 3, respectively), and the second is called the \emph{octupolar} Hamiltonian (following the terminology of electrostatic multipoles). Since $\tilde{\sigma}_{j,2}=1$ for $j=1,2$, we write
\begin{equation}\label{eq_sechamexpansion}
F_{\mathrm{sec}}^{j,j+1}= - \frac{\mu_j \, m_{j+1}}{(2 \pi)^2} \left( F_{\mathrm{quad}}^{j,j+1} + \tilde{\sigma}_{j,3} \, F_{\mathrm{oct}}^{j,j+1} + O \left( \frac{ a_j^4}{a_{j+1}^5} \right) \right)
\end{equation}
for $j=1,2$. The eccentricity of the $j^{\mathrm{th}}$ Keplerian ellipse is given in terms of Deprit coordinates by
\begin{equation} \label{eq_eccentricity}
e_j = \sqrt{1 - \frac{\Gamma_j^2}{L_j^2}}.
\end{equation}

\begin{lemma}\label{lemma_quadoct12comp}
The quadrupolar and octupolar Hamiltonians of bodies 1 and 2 are given by
\begin{equation} \label{eq_quad12unscaled}
F_{\mathrm{quad}}^{12}= \frac{a_1^2}{8 \, a_{2}^3 \, (1-e_{2}^2)^{\frac{3}{2}}} \left( \left( 15 \, e_1^2 \cos^2 \gamma_1 - 12 \, e_1^2 - 3 \right) \sin^2 i_{12} + 3 e_1^2 + 2 \right)
\end{equation}
and 
\begin{equation} \label{eq_oct12unscaled}
\begin{split} 
F_{\mathrm{oct}}^{12} ={}& - \frac{15}{64} \frac{a_1^3}{a_2^4} \frac{e_1 \, e_2}{\left(1 -e_2^2 \right)^{\frac{5}{2}}} \\
& \times \left\{
\begin{split}
\cos \gamma_1 \, \cos \gamma_2 \left[
\begin{split}
\frac{\Gamma_1^2}{L_1^2} \left(5 \, \sin^2 i_{12} \left(6-7 \cos^2 \gamma_1 \right) - 3 \right) \\
-35 \, \sin^2 \gamma_1 \, \sin^2 i_{12} + 7
\end{split}
\right] \\
+ \sin \gamma_1 \, \sin \gamma_2 \, \cos i_{12} \left[
\begin{split}
\frac{\Gamma_1^2}{L_1^2} \left(5 \, \sin^2 i_{12} \left(4 - 7 \, \cos^2 \gamma_1 \right) - 3 \right) \\
- 35 \sin^2 \gamma_1 \, \sin^2 i_{12} + 7
\end{split}
\right]
\end{split}
\right\} 
\end{split}
\end{equation}
respectively, where $e_j$ is the eccentricity of the $j^{\mathrm{th}}$ Keplerian ellipse, and $i_{12}$ is the mutual inclination of Keplerian bodies $1$ and $2$, defined by
\begin{equation}\label{eq_cosi12def}
\cos i_{12} = \frac{\Gamma_1^2 + \Gamma_2^2 - \Psi_1^2}{2 \, \Gamma_1 \, \Gamma_2}.
\end{equation}
\end{lemma}
\begin{proof}
The quadrupolar and octupolar Hamiltonians are defined by
\begin{equation}
F_{\mathrm{quad}}^{12} = \int_{\mathbb{T}^2} P_2 \left( \cos \zeta_{1} \right) \frac{\| q_1 \|^2}{\| q_2 \|^3} \, d \ell_1 \, d \ell_{2}, \quad F_{\mathrm{oct}}^{12} = \int_{\mathbb{T}^2} P_3 \left( \cos \zeta_{1} \right) \frac{\| q_1 \|^3}{\| q_2 \|^4} \, d \ell_1 \, d \ell_{2}.
\end{equation}
In order to measure $\cos \zeta_1$, it is sufficient to derive expressions for $q_1,q_2$ in Deprit coordinates with respect to any orthonormal basis of $\mathbb{R}^3$. Recall the definition of the nodes $\nu_i$. As in Claim 1 of \cite{chierchia2011deprit} we consider the \emph{orbital basis} $B_i = (k_{i,1},k_{i,2},k_{i,3})$ for $i=1,2$, where
\begin{equation}
k_{i,1} = \frac{\nu_i}{\| \nu_i \|}, \quad k_{i,3} = \frac{C_i}{\| C_i \|},
\end{equation}
and where $k_{i,2}$ is chosen to make the basis orthonormal. We assume that $q_i \in \mathbb{R}^3 \setminus \{ 0 \}$. Let $\bar{q}_i = \| q_i \|^{-1} q_i$. Then, by the definition of the angle $\gamma_i$, the point $\bar{q}_i$ is written with respect to $B_i$ as $\bar{Q}_i=(\cos (\gamma_i+v_i), \sin (\gamma_i + v_i), 0)$, where $v_i$ is the true anomaly corresponding to the mean anomaly $\ell_i$. Define the standard rotation matrix by an angle $\theta \in \mathbb{T}$ around the $x$-axis by
\begin{equation}
\R_1 (\theta) = \left(
\begin{matrix}
1 & 0 & 0 \\
0 & \cos \theta & - \sin \theta \\
0 & \sin \theta & \cos \theta 
\end{matrix}
\right).
\end{equation}
Since $\nu_1=\nu_2$, the change of basis matrix from $B_1$ to $B_2$ is $\R_1 (i_{12})$, and so
\begin{equation}
\cos \zeta_1 = \R_1 (i_{12}) \bar{Q}_1 \cdot \bar{Q}_2.
\end{equation}
A standard computation (see Appendix C of \cite{fejoz2002quasiperiodic}; compare also equations (6), (7) of \cite{fejoz2016secular}) completes the proof.
\end{proof}

\begin{remark}
We can obtain similar expressions for the quadrupolar and octupolar Hamiltonians of bodies 2 and 3. However these expressions rely on a change of variables, and a Taylor expansion in these new variables. This coordinate transformation and expansion is carried out in the next section. 
\end{remark}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "4bp_secular_diffusion_v4.tex"
%%% End: 

